Emergence of Scenario-Appropriate Collaborative Behaviors for Teams of Robotic Bodyguards

We are considering the problem of controlling a team of robotic bodyguards protecting a VIP from physical assault in the presence of neutral and/or adversarial bystanders. This task is part of a much larger class of problems involving coordinated robot behavior in the presence of humans. This problem is challenging due to the large number of active entities with different agendas, the need of cooperation between the robots as well as the requirement to take into consideration criteria such as social norms and unobtrusiveness in addition to the main goal of VIP safety. Furthermore, different settings such as street, public space or red carpet require very different behavior from the robot. We describe how a multi-agent reinforcement learning approach can evolve behavior policies for teams of robot bodyguards that compare well with hand-engineered approaches. Furthermore, we show that an algorithm inspired by universal value function approximators can learn policies that exhibit appropriate, distinct behavior in environments with different requirements.

==> RewardFunctions.tex <==
\subsection*{Reward Functions}
\label{sec:RewardFunctions}

In~\cite{Bhatia-2016-FLAIRS} has defined a metric that quantifies the threat to the VIP from each crowd member $b_{i}$ at each timestep $t$. This metric can be extended to a reward function. Since the threat level metric gives a probability. We can conclude that when the distance between the VIP and the crowd member is 0, the threat to the VIP is maximum, i.e 1, conversely when the distance between the VIP and the crowd member $b_{i}$ is more than the \textit{safe distance}, the threat to the VIP is 0. We can model this phenomenon as an exponential decay.
In the following we will derive reward function and explain the motivation behind them that were derived from~\cref{eq:crt}.

The baseline {\em Threat-Only Reward Function} penalizes each agent with the threat to the VIP at each time step as mentioned in~\cite{Bhatia-2016-FLAIRS}.
\begin{equation}
r_{g} =-1+\prod_{i=1}^{k}\left(1-\mathit{RT}\left(VIP,b_{i}, R\right)\right)
\label{eq:ThreatOnly}
\end{equation}

%\subsubsection{Composite Reward Function}
The {\em Composite Reward Function} is the composition of the threat only reward function and the penalty for not maintaining a suitable distance from the VIP.

\begin{equation}
\mathcal{D}\left(\mathit{VIP},x_{i}\right)=\begin{cases}
0 & m \leq\left\Vert x_{i}-\mathit{VIP}\right\Vert _{2}\leq d\\
-1 & \text{otherwise}\\
\\
\end{cases}
\end{equation}

\noindent where $m$ is the minimum distance the bodyguard has to maintain from VIP and $d$ is the safe distance.  The final reward function is represented as

\begin{equation}
\begin{aligned}
r_{g}  =&\alpha\left(\displaystyle -1+\prod_{i=1}^{k}\left(1-\mathit{RT}\left(VIP,b_{i}, R\right)\right) \right) \\&
+\beta\left( \mathcal{D}\left(\mathit{VIP},x_{i}\right)\right)
\end{aligned}
\label{eq:Composite}
\end{equation}

Each scenario $g$ has different values of $\alpha, \beta$ and $m$, thus fulfilling the requirement of different goals having different reward structure.

In this problem, we are assuming that all bodyguards have identical observation space and action space. For this problem we are considering a finite horizon setting where each episode is terminated after \textbf{T} steps. Since this problem is a cooperative setting, the goal of the agents is to find individual policies that increase the collected payoff.

